Human-AI collaboration is not very collaborative yet: A taxonomy of interaction patterns in AI-assisted decision making from a systematic review

Leveraging Artificial Intelligence (AI) in decision support systems has disproportionately focused on technological advancements, often overlooking the alignment between algorithmic outputs and human expectations. A human-centered perspective attempts to alleviate this concern by designing AI solutions for seamless integration with existing processes. Determining what information AI should provide to aid humans is vital, a concept underscored by explainable AI's efforts to justify AI predictions. However, how the information is presented, e.g., the sequence of recommendations and solicitation of interpretations, is equally crucial as complex interactions may emerge between humans and AI. While empirical studies have evaluated human-AI dynamics across domains, a common vocabulary for human-AI interaction protocols is lacking. To promote more deliberate consideration of interaction designs, we introduce a taxonomy of interaction patterns that delineate various modes of human-AI interactivity. We summarize the results of a systematic review of AI-assisted decision making literature and identify trends and opportunities in existing interactions across application domains from 105 articles. We find that current interactions are dominated by simplistic collaboration paradigms, leading to little support for truly interactive functionality. Our taxonomy offers a tool to understand interactivity with AI in decision-making and foster interaction designs for achieving clear communication, trustworthiness, and collaboration.

==> background.tex <==
\subsection{Humans in decision-making} 
Decision-making is the selection of an action within discrete choices, usually guided by multiple factors, such as rationality, emotion, experience, intuition, and heuristics~\cite{redish2013mind,gigerenzer2008heuristics}. With multiple factors to consider, human decision-making can be affected by cognitive biases that impair information processing~\cite{oeberst2023toward}. A common framework to understand human decision-making is the dual process model, which distinguishes between fast and intuitive (System 1) and slow and logical (System 2) cognitive processes~\cite{Kahneman11}. System 1 can be efficient but error-prone due to simplifications or quick assessments (also known as heuristics), while System 2 can be more accurate but costly. 
Understanding human decision making processes can inform the design of AI systems that complement human strengths and mitigate weaknesses as they make decisions. It further informs the design of user interfaces that afford certain interaction mechanisms, e.g., depending on the presentation and framing of information and incorporation of user feedback. Research on interaction mechanisms can provide insights to mitigate biases in human decision making and improve the outcomes as humans collaborate with AI.
% AI recommendations can provide System 2-like support offering data-driven and logical analysis, to potentially reduce errors and biases, and improve efficiency. Human-AI systems can leverage the strengths of both systems to enhance decision quality and outcomes.}
% connection between biases and AI: biases might arise when presented recommendations from AI due to human interpretation 

Moreover, many human decisions are not made in isolation but in collaboration with others who may have different perspectives, opinions, or expertise. Collaboration can enhance decision-making by providing access to more information, diverse viewpoints, and constructive feedback~\cite{bahrami2010optimally}. However, collaboration may introduce costs and challenges, such as coordination difficulties, social influence, group thinking, or conflict~\cite{minson2012cost}. Therefore, it is important to understand how humans incorporate others’ advice in their decision-making process, and under what conditions collaboration can improve or impair judgment quality. Several factors can change one's initial judgment after receiving advice from another person, such as the perceived credibility of the advisor, the similarity or dissimilarity of the initial judgments, the type and format of the advice, and the motivation and personality of the decision maker~\cite{gino2008take}. Human collaboration provides workflows and insights for studying human-AI interaction because it can inform the design and evaluation of AI systems to provide effective and trustworthy advice to humans.

\subsection{AI integration in decision making}
% 1. what can AI do for humans: support or replace decision makers? In low-stakes? e.g., recommender systems. high-stakes domains? e.g., decision aids. 
% 2. how does it support decision making. E.g., what is provided to people? how? 
% 3. What are observed challenges here? e.g., overreliance, algorithmic aversion

%% TODO: add and connect all these references
% categories of AI system applications~\cite{duan2019artificial}
% roles that AI automation can fulfil~\cite{leon2021accountability}. AI can operate with different degrees of autonomy (e.g., partial or conditional autonomy)

% Guidelines human-AI interactions\cite{amershi2019guidelines} 

% cooperation between humans and machines~\cite{haesevoets2021human}. Importance of trust and acceptance. 

% levels of Automation (LoA) showing possible interactions between human and computer \cite{Mackeprang2019-dz}

% Identify tasks performed by the AI, human or both. how much initiative, agency, or authority each party has at each step~\cite{muller2022extending}

% roles of human-AI team members in the interaction~\cite{tsiakas2022using}
% AI used to augment~\cite{miller2018ai}


%~\cite{van2023measurements} describes interactions with AI decision support tools in medical use cases and references to user studies that evaluate AI as decision support 
%~\cite{sheu2022survey}
Artificial intelligence developments provide solutions to perform tasks that normally require human intelligence, such as perception, reasoning, learning, decision making, and problem solving~\cite{duan2019artificial}. AI has been applied to various domains and contexts, ranging from low-stakes to high-stakes, where human decision-making is involved or affected~\cite{duan2019artificial}. Depending on the level of autonomy and authority that AI has in the decision-making process, AI can play different roles for humans: support human decision making by providing information, suggestions, or feedback that can help humans make better or faster decisions; augment human decision making by performing some tasks that are too complex, tedious, or risky for humans, while still allowing humans to have control or oversight over the final decisions; replace human decision making by taking over the entire responsibility and accountability for the decisions and actions, without requiring human intervention or approval~\cite{leon2021accountability}. Overall, AI provides novel ways of human-machine interaction and emerging aspects that require further investigation.

Similar to collaborations in human decision-making, ensuring effective cooperation between humans and machines also has many challenges. Cooperation requires trust and acceptance from both parties, which depend on factors such as transparency, explainability, accuracy, fairness, and ethics of the AI system~\cite{haesevoets2021human}. Another challenge is balancing the level of automation and human involvement in the decision-making process. Too much automation can lead to over-reliance or complacency from humans, who may lose their skills or situational awareness due to reduced cognitive load or feedback~\cite{Mackeprang2019-dz}.  Too little automation can lead to algorithmic aversion or resistance from humans, who may distrust or disregard the AI system due to perceived errors or biases~\cite{sheu2022survey}.
Thus, the amount of automation provided by AI directly affects human actions and their sense of agency, which are later reflected in different human behaviors. Understanding different factors that shape interactions is crucial for selecting design elements that best fit a scenario that integrates AI in decision making. Thinking about human-AI interactions from the early development of AI solutions and iterating continuously over design choices follows a human-centered approach to AI, in which developers reach to end users and their contexts, as it has been the case of building explainable AI in the medical domain~\cite{chen2022explainable,van2023measurements}.


% In high-risk decision-making areas like medical applications, research on human-AI interaction can help ensure that AI systems are designed with human needs and context requirements in mind. However, most of the research in the medical domain focuses on the technical and algorithmic developments~\cite{chen2022explainable,van2023measurements}.  
% One effort to build trust between users and AI systems is to develop medical explainable AI (XAI)~\cite{sheu2022survey}. Aside from just focusing on the presentation of the AI systems, the misalignment between medical end-users and AI researchers and developers can be better overcome by thinking about human-AI interactions from the early development of AI solutions and iterating over design choices~\cite{van2023measurements}.
% AI has been used in medicine for various purposes such as diagnosis, treatment, and drug discovery. For example, by analyzing large amounts of data from clinical trials, AI can help clinicians identify which patients are most likely to benefit from a particular treatment. This can help to improve the effectiveness of treatments and reduce the risk of side effects. In general, research on human-AI interaction in the medical domain is important because it can help ensure that AI systems are designed with human needs in mind. This is especially important in high-risk decision-making areas like medical applications. However, most of the research in the medical domain focuses on the technical side and the algorithms. Although we observed a surge in the introduction of AI decision-making tools, we also saw the disappearance of end-users’ ability to validate a system’s performance \cite{van2023measurements}. 

%Another previous work provides a survey of recent progress in medical explainable AI (XAI) \cite{sheu2022survey}. The authors discuss the importance of human-AI interaction in the medical domain and argues that explainability is crucial in building trust between users and AI systems. Aside from just focusing on the presentation of the AI systems, Berkel \cite{van2023measurements} aims to overcome this misalignment between medical end-users and AI researchers and developers by defining Human-AI interaction across three stages: Measurement, Algorithm, and Presentation. They identified the challenges faced by each stage by referencing user studies and provided suggestions on improvements.

\subsection{Surveys in human-AI interaction}
The growing interest to augment human decision-making with AI assistance has been captured by surveys focused on human-AI interactions studies.  
A recent survey started by characterizing what the community defines as human-centered AI and how these claims are related to the interaction with AI~\cite{capel2023human}. This definition comprises approaches to design and evaluate AI, humans teaming with AI, ethical AI, and a new emerging area of interaction design that investigates how people interact with AI systems and how AI is represented in the user interface.
An overview of human-AI decision-making studies identified trends in different aspects of the design space in empirical works, suggesting more careful consideration and justification of tasks and evaluation metrics~\cite{oeberst2023toward}. Another aspect more closely related to interactions examined AI assistance elements, namely the type of model predictions, support information and interventions or workflows, as these ultimately allow for interactions with a user. Only a few examples were used to illustrate different levels of user control or machine agency.
% decision making tasks: more careful consideration and justification of tasks 
% extracted information on AI assistance elements - dictate and affect the interactions enabled. type of predictions, information about predicitons or about the model, interventions (workflow, barely touch and provide some examples of user control-guide the model output, control over explanations, machine agency)   
% evaluation: what to evaluate and how to evaluate the target construct. Separate it by those related to the task or the AI. Here we analyze them by domains. Common/standard metrics -> development of common frameworks for human-AI decision making.    
% goal of the survey: provide recommendations for practices in designing and conducting these studies, including different aspects of the design space (task, AI assistance elements, evaluation)
As the concept of trust is critical in AI-embedded systems, previous surveys have characterized the experimental protocols used to evaluate trust and provided practical guidelines~\cite{vereschak2021evaluate}.
Other surveys have suggested taxonomies to organize human-AI studies across multiple dimensions, including components related to the interactions with AI. For instance, the complementing flow in the human-AI team determines the interactions that can take place~\cite{zahedi2021human}, i.e., the human can provide inputs to improve the AI system or the AI can make it results understandable, while bidirectional complementing requires communications or actions from both agents and their cooperation as such. Furthermore, the teaming goal can be affected by the interaction state. The human and machine part of the interaction was analyzed separately considering factors unique to each one, such as the amount and type of human input, or the AI's feedback to humans and interpretability ~\cite{dellermann2021future}.
Another survey identified factors that influence collaboration between humans and AI, especially the utility of explanations to achieve better team outcomes\cite{hemmer2021human}. Collaboration characteristics included the degree of automation, the order in which predictions and explanations are made available, and the interactivity of the system, although the discussion was limited to a use case when explanations are adaptive. Recommendations for future research suggested to actively involve the human in the decision making process, resulting in dynamic interactions, such as delegation or choosing to reveal the AI recommendations; both observed in the studies within our survey.
% goal of the survey: organize human-AI works based on different dimensions
% \new{Related factors, such as teaming goals and task horizon, compose the dimensions of another taxonomy of recent works in human-AI teams~\cite{zahedi2021human}. Another dimension within this taxonomy considers the complementing flow in the team as it determines the interactions that can take place. For example, the human providing inputs to improve the AI system or making the AI understandable result in one agent complementing the other, while bidirectional complementing requires communications or actions from both agents and their cooperation as such.}
% teaming goal (affected by the interaction state, whether single or multiple interactions, e.g., seeking for immediate rewards in the former).
% Need for structured design knowledge for building systems that combine human and AI. research on the role of humans in the ML pipeline, resulting in hybrid intelligence systems. Propose a taxonomy for system design/development, that includes a dimension for human-AI (amount of human input, explicit and implicit teaching) and AI-human interaction (feedback to human, learning strategy that affects human teaching, interpretability), plus task characteristics and learning paradigm~\cite{dellermann2021future}
% identify factors that influence collaboration between humans and AI, focused on hybrid intelligence systems that leverage XAI as a collaboration mechanism, and the utility of explanations to achieve complementary team performance or on relevant behavioral constructs \cite{hemmer2021human}
% only 29 articles that conducted empirical research, extracted the treatments into four groups: 
% collaboration: order in which predictions and explanations are made available to humans and interactivity of the HI system, degree of automation  
% task, AI, and human characteristics: skill sets and data type, XAI techniques and implementations, presentation of information, human knowledge of AI 
% other factors of the to consider: actively involve the human in the decision making process: dynamic interactions, make decisions on their own before, let the user decide what they want to see (request), delegation. All related to the interaction with AI/collboration. Difference in performance with AI 
As the emerging field of XAI constitutes a large portion of human-AI interaction studies, previous surveys have focused on explainability in human-AI interaction\cite{chen2022explainable,bertrand2022cognitive,bertrand2023selective}. These surveys have provided a comprehensive description of different explainable AI components, such as existing explainability techniques and evaluation approaches used in the medical domain~\cite{chen2022explainable}, cognitive biases that affect or are affected by XAI systems~\cite{bertrand2022cognitive}, and user evaluations of interactive explanations~\cite{bertrand2023selective}. In addition, the latter created a classification of interactive techniques specific to XAI and grouped the resulting categories according to their role in the cognitive process of explanation: “selective”, “mutable” or “dialogic”. Selective techniques help users filter out irrelevant information, mutable techniques help users modify the AI model or its inputs, and dialogic techniques help users engage in a conversation with the AI system. 
% only considers explanations that were meant to be interactive
% human and AI considered separately, but the interaction is the occurrence of both. 

We expanded the characterization of interactivity beyond the functions that explanations can provide and integrated the human and machine parts of the interaction together, which allowed us to consider the full picture of incorporating AI systems as decision support. In this way, our classification of interaction patterns covers other factors such as the type of assistance that AI can provide and when it is presented to the users during their interaction.   



\subsection{Interaction patterns}
Understanding interactions requires delving into multiple dimensions that involve subjects, modes, and purposes of interaction, and the context in which they take place~\cite{schleidgen2023concept}.
Among these, interaction patterns emerge as sequences of behaviors that occur more often than by chance between agents and systems or artifacts. For purposes of this work, studying interaction patterns can help researchers understand how humans and AI can work together and design systems that are easy to use and achieve the intended goals.
Psychology and social sciences have extensively studied human-human interactions, revealing patterns of reciprocal actions, such as "Question-Answer" and "Request-Offer"~\cite{magnusson_2018}, which can also be applied in a setup where humans interact with AI. For example, when an AI system provides answers to the user’s questions or asks questions to elicit the user’s preferences or feedback. 
Likewise, the field of Human-Robot Interaction (HRI) has studied how humans and robots communicate, collaborate, and engage with each other, often through the analysis of observable patterns in their interactions. Researchers have created templates and libraries for programming and designing human-robot interactions, using building blocks of interaction as interaction design patterns ~\cite{david2022interaction,sauppe2014design,ma2019design}. These patterns cover various aspects of social interactions, such as greetings, attention, feedback, turn-taking, social cues, and farewell. All these elements foster a more natural and efficient communication experience, which can take place in AI technologies that incorporate natural language abilities. 
Other domains such as information visualization and user interface design have also developed taxonomies and libraries of interaction patterns based on different criteria such as user’s intent, purpose, scope, abstraction level, and granularity \cite{yi2007toward,silva2020classifying}. These criteria help designers to understand the characteristics and relationships of different design patterns and choose the most suitable ones for the systems they are building.

In the context of human-AI interaction, one way to classify interactions is by frequency: intermittent (occasional interactions), continuous (more frequent interactions), and proactive (led by AI's initiative)~\cite{van2021human}. Another way to classify interactions is by autonomy: human-dominated, machine-dominated, or balanced~\cite{xiong2023partner}. Human-dominated interaction refers to situations where machines act as an aid and humans retain the final right to make decisions. Machine-dominated interaction refers to situations where machines act as an authority and humans follow their instructions. Balanced interaction refers to situations where machines act as a partner and humans share decision-making power. A third way to classify interactions is by task complexity: simple (routine or repetitive tasks), moderate ( partially defined and uncertain tasks), or complex (ill-defined and dynamic tasks)~\cite{parasuraman2000model}. Decision-making workflows can further result in different interaction paradigms: a sequential one where AI advice follows the human’s initial independent judgment, allowing for subsequent revisions, and a concurrent one when AI advice is presented alongside the prediction problem \cite{tejeda2022ai}. Similarly, a survey grouped interaction flows into four types of decision making processes that basically differ by the presentation of recommendations~\cite{vereschak2021evaluate}. As this categorization was proposed by a survey concerned with the empirical evaluation of trust, the analysis of interaction flows was associated with behavioral metrics that can be calculated for each one.
% Observation: studies do not motivate their choice of the interaction flow}. 
A synthesis of types of interactions explored in prior works on AI-assisted text generation informed the definition of a taxonomy that is primarily structured around human actions and the extent of their control over the final text output~\cite{cheng2022mapping}. User interviews evaluating the experience with these different types of interactions underscored the trade-offs between maintaining control and achieving task efficiency.
% ~\cite{cheng2022mapping}, understand human roles when interacting or being assisted by AI in text generation tasks. Developed a taxonomy of interactions in AI-assisted text generation informed by a systematic review organized by human actions, controls (over the AI output), workflows (who initiates), and interfaces from the literature (very specific to text features, words, sentences). Synthesize types of interactions explored in prior work. Used the taxonomy to explore user needs and experience with these interactions through an interview user study. identify trade-offs between control and task efficiency, need for customizable timing of control, avoid disruptions  
% Importance of having a taxonomy when designing new systems or experiments to select the interaction and design elements that best fit the scenario, and gain a more formal understanding by being able to compare findings to prior works. 
% ours: taxonomy for broader set of decision making tasks and includes actions of both the human and AI, also the visualizations display the order in the workflow of the interaction. 

Overall, the existing classifications of interactions that involve AI are mostly focused on specific domains or contexts but do not provide a general and comprehensive framework for characterizing and analyzing interaction patterns that apply to multiple domains. % and are supported by empirical evidence
The dimensions of frequency, autonomy, complexity, workflows, and human actions can be combined to form an extensive taxonomy of human-AI interaction patterns. 
Combining insights and principles from interaction patterns in other disciplines and the findings from our systematic review, in this work we take a first step to provide a common vocabulary to describe human-AI interaction patterns in a broader set of decision making tasks.  

